Camouflage is all you need: Evaluating and Enhancing Language Model Robustness Against Camouflage Adversarial Attacks

Adversarial attacks represent a substantial challenge in Natural Language Processing (NLP). This study undertakes a systematic exploration of this challenge in two distinct phases: vulnerability evaluation and resilience enhancement of Transformer-based models under adversarial attacks. In the evaluation phase, we assess the susceptibility of three Transformer configurations, encoder-decoder, encoder-only, and decoder-only setups, to adversarial attacks of escalating complexity across datasets containing offensive language and misinformation. Encoder-only models manifest a 14% and 21% performance drop in offensive language detection and misinformation detection tasks, respectively. Decoder-only models register a 16% decrease in both tasks, while encoder-decoder models exhibit a maximum performance drop of 14% and 26% in the respective tasks. The resilience-enhancement phase employs adversarial training, integrating pre-camouflaged and dynamically altered data. This approach effectively reduces the performance drop in encoder-only models to an average of 5% in offensive language detection and 2% in misinformation detection tasks. Decoder-only models, occasionally exceeding original performance, limit the performance drop to 7% and 2% in the respective tasks. Although not surpassing the original performance, Encoder-decoder models can reduce the drop to an average of 6% and 2% respectively. Results suggest a trade-off between performance and robustness, with some models maintaining similar performance while gaining robustness. Our study and adversarial training techniques have been incorporated into an open-source tool for generating camouflaged datasets. However, methodology effectiveness depends on the specific camouflage technique and data encountered, emphasizing the need for continued exploration.

==> table_camouflaged_examples.tex <==
\begin{table}[]
\caption{Comparison of original and camouflaged text examples from the Offen SemEval 2019 and Constraint datasets. The table presents examples of three levels of camouflage by the tool introduced in this study, as well as an example from the AugLy library for external validation with unseen modifications. Each level represents increasing complexity of camouflage.}
\label{table:data-example}
\vspace{1mm}
\fontspec{DejaVu Sans} % Set the font to DejaVu Sans only for the table
\renewcommand{\arraystretch}{1.5} % Add this line to increase row spacing

\begin{tabularx}{\textwidth}{lXX} % Use tabularx with the width set to \textwidth, and adjust column widths using 'X'
\toprule
                  & \multicolumn{1}{c}{\textbf{Offen SemEval}}                                                                                  & \multicolumn{1}{c}{\textbf{Constraint}}                                                                                                                                            \\ 
\hline
\textbf{Original} & 6 ANTIFA ATTACKED COPS, ARRESTED
AT RALLY IN DENVER, MEDIA BLACKOUT URL                                                     & FDA
chief Hahn comments about convalescent plasma for \#COVID-19 patients stirred
controversy and a shake up at the agency.                                                        \\ 
\hline
\textbf{Level 1}  & 6 ANTįFA ATTACKED CʘPS, ăRRƸST3D AT RALLY IN DēNVėR, MEDĩ∀ BLACKOUT URL                                                     & FDą ch!ěf Hahn comments about convalescent plasma for \#COVID-19 pȁtïƸnts stirred controversy and a shake up at the ∀gency.                                                       \\ 
\hline
\textbf{Level 2}  & 6 Aͷ'T1FA ATTACKED :ć:O:P:ś:,
āR]RͼϟTͼĐ AT RALLY IN \textbar{})ƐN;VƐR, ɱĕĐ!@ BLACKOUT
URL~ ~ ~                              & \%F\%D\%A~ cĥįȇf \textbar{}-\textbar{}Ʌhℕ~ comments about convalescent plasma for
\#CȱVID-19 \_\textbar{}\_>\_a\_t\_i\_Ɛ\_n\_t\_s stirred controversy and a shake up at the
Ƌgeͷcy  \\ 
\hline
\textbf{Level 3}  & 6@Д@η@ȶ@į@ſ@Д ATTACKED COPS, ąR\textgreater{}RℯSTƸđAT RALLY IN DēN√ēR, [)1A]V[E BLACKOUT URL                                & /=(\textbar{}ä'ch][Ə'f Ha'hn c'omme'nts 'abou't co'nval'esce'nt p'lasm'a fo'r \#C'OVID'-19 ℙⱥŦïěnŦs sti'rred' con'trov'ersy' and' a s'hake' up 'at t'he ~a g ƹ n č y.              \\ 
\hline
\textbf{AugLy}    & 6
AN...ṫIFA... ATT...ACKE...D CO...PS, ...AŕRE...STEȡ... AT ...RẰLL...Y IN...
DEN...VER,... MED...IA B...L@CK...OU7 ...U/2L & FDA chief Hahn ĆommenṮs about convalescent plasma foℜ\#CO∨ID-19 patients stiɌrĒd controversy and a shake uƿ aț the agency.                                                         \\
\bottomrule
\end{tabularx}
\fontspec{Times New Roman}
\end{table}
